Multiwavelength observations of nova SMCN 2016-10a --- one of the brightest novae ever observed

We report on multiwavelength observations of nova SMCN 2016-10a. The present observational set is one of the most comprehensive for any nova in the Small Magellanic Cloud, including: low, medium, and high resolution optical spectroscopy and spectropolarimetry from SALT, FLOYDS, and SOAR; long-term OGLE $V$- and $I$- bands photometry dating back to six years before eruption; SMARTS optical and near-IR photometry from $\sim$ 11 days until over 280 days post-eruption; $Swift$ satellite X-ray and ultraviolet observations from $\sim$ 6 days until 319 days post-eruption. The progenitor system contains a bright disk and a main sequence or a sub-giant secondary. The nova is very fast with $t_2 \simeq$ 4.0 $\pm$ 1.0 d and $t_3 \simeq$ 7.8 $\pm$ 2.0 d in the $V$-band. If the nova is in the SMC, at a distance of $\sim$ 61 $\pm$ 10 kpc, we derive $M_{V,\mathrm{max}} \simeq - 10.5$ $\pm$ 0.5, making it the brightest nova ever discovered in the SMC and one of the brightest on record. At day 5 post-eruption the spectral lines show a He/N spectroscopic class and a FWHM of $\sim$ 3500 kms$^{-1}$ indicating moderately high ejection velocities. The nova entered the nebular phase $\sim$ 20 days post-eruption, predicting the imminent super-soft source turn-on in the X-rays, which started $\sim$ 28 days post-eruption. The super-soft source properties indicate a white dwarf mass between 1.2 M$_{\odot}$ and 1.3 M$_{\odot}$ in good agreement with the optical conclusions.

==> journal.tex <==
 \newcommand*\aap{A\&A}
\let\astap=\aap
\newcommand*\aapr{A\&A~Rev.}
\newcommand*\aaps{A\&AS}
\newcommand*\actaa{Acta Astron.}
\newcommand*\aj{AJ}
\newcommand*\ao{Appl.~Opt.}
\let\applopt\ao
\newcommand*\apj{ApJ}
\newcommand*\apjl{ApJ}
\let\apjlett\apjl
\newcommand*\apjs{ApJS}
\let\apjsupp\apjs
\newcommand*\aplett{Astrophys.~Lett.}
\newcommand*\apspr{Astrophys.~Space~Phys.~Res.}
\newcommand*\apss{Ap\&SS}
\newcommand*\araa{ARA\&A}
\newcommand*\azh{AZh}
\newcommand*\baas{BAAS}
\newcommand*\bac{Bull. astr. Inst. Czechosl.}
\newcommand*\bain{Bull.~Astron.~Inst.~Netherlands}
\newcommand*\caa{Chinese Astron. Astrophys.}
\newcommand*\cjaa{Chinese J. Astron. Astrophys.}
\newcommand*\fcp{Fund.~Cosmic~Phys.}
\newcommand*\gca{Geochim.~Cosmochim.~Acta}
\newcommand*\grl{Geophys.~Res.~Lett.}
\newcommand*\iaucirc{IAU~Circ.}
\newcommand*\icarus{Icarus}
\newcommand*\jcap{J. Cosmology Astropart. Phys.}
\newcommand*\jcp{J.~Chem.~Phys.}
\newcommand*\jgr{J.~Geophys.~Res.}
\newcommand*\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}
\newcommand*\jrasc{JRASC}
\newcommand*\memras{MmRAS}
\newcommand*\memsai{Mem.~Soc.~Astron.~Italiana}
\newcommand*\mnras{MNRAS}
\newcommand*\na{New A}
\newcommand*\nar{New A Rev.}
\newcommand*\nat{Nature}
\newcommand*\nphysa{Nucl.~Phys.~A}
\newcommand*\pasa{PASA}
\newcommand*\pasj{PASJ}
\newcommand*\pasp{PASP}
\newcommand*\physrep{Phys.~Rep.}
\newcommand*\physscr{Phys.~Scr}
\newcommand*\planss{Planet.~Space~Sci.}
\newcommand*\pra{Phys.~Rev.~A}
\newcommand*\prb{Phys.~Rev.~B}
\newcommand*\prc{Phys.~Rev.~C}
\newcommand*\prd{Phys.~Rev.~D}
\newcommand*\pre{Phys.~Rev.~E}
\newcommand*\prl{Phys.~Rev.~Lett.}
\newcommand*\procspie{Proc.~SPIE}
\newcommand*\qjras{QJRAS}
\newcommand*\rmxaa{Rev. Mexicana Astron. Astrofis.}
\newcommand*\skytel{S\&T}
\newcommand*\solphys{Sol.~Phys.}
\newcommand*\sovast{Soviet~Ast.}
\newcommand*\ssr{Space~Sci.~Rev.}
\newcommand*\zap{ZAp}
